Correlation Clustering with Asymmetric Classification Errors

In the Correlation Clustering problem, we are given a weighted graph $G$ with its edges labeled as "similar" or "dissimilar" by a binary classifier. The goal is to produce a clustering that minimizes the weight of "disagreements": the sum of the weights of "similar" edges across clusters and "dissimilar" edges within clusters. We study the correlation clustering problem under the following assumption: Every "similar" edge $e$ has weight $\mathbf{w}_e\in[\alpha \mathbf{w}, \mathbf{w}]$ and every "dissimilar" edge $e$ has weight $\mathbf{w}_e\geq \alpha \mathbf{w}$ (where $\alpha\leq 1$ and $\mathbf{w}>0$ is a scaling parameter). We give a $(3 + 2 \log_e (1/\alpha))$ approximation algorithm for this problem. This assumption captures well the scenario when classification errors are asymmetric. Additionally, we show an asymptotically matching Linear Programming integrality gap of $\Omega(\log 1/\alpha)$.

==> prf-triangle-just.tex <==
\section{Proof of Theorem~\ref{thm:L4}}
\noindent\textbf{\color{red} Remark: } {\color{red} Previous version(to be removed)}

For the sake of completeness we include the proof of Theorem~\ref{thm:L4} (see \cite{ACN08} and \cite{CMSY15})

\begin{proof}[Proof of Theorem~\ref{thm:L4}]
Consider a function $f$ with $f(0) = 0$. We prove that if for all signatures $\sigma=(\sigma_1,\sigma_2,\sigma_3)$ (where each $\sigma_i\in \{\pm\}$) and edge lengths $x$, $y$, and $z$ satisfying the triangle inequality, we have $ALG^{\sigma}(x,y,z)\leq \rho LP^{\sigma}(x,y,z)$, then the approximation factor of Algorithm~\ref{alg:ApprAlg} is at most $\rho$.


Consider step $t$ of the algorithm. Let the set of active vertices denoted by $V_t$ and $w\in V_t$ be a pivot chosen at step $t$. The algorithm chooses a set $S_t \subseteq V_t$ and removes it from the graph. Notice that if $u \in S_t$ or $v \in S_t$, then the constraint imposed by $(u,v)$ is
satisfied or violated right after step $t$. Specifically, if $(u,v)$ is a positive edge, then the constraint $(u,v)$ is violated if exactly one of the vertices $u,v$ is in $S_t$. If $(u,v)$ is a negative constraint, then it is violated if both $u,v$ are in $S_t$. Denote the total weight of violated constraints at step $t$ by $ALG_t$. Then,

\begin{align*}
ALG_t=&\sum\limits_{\substack{(u,v) \in E^+\\u,v \in V_t}} w_{uv}\cdot\ONE \left(u \in S_t, v \not\in S_t \mbox{ or }u \not\in S_t, v \in S_t\right)\\
&+\sum\limits_{\substack{(u,v) \in E^-\\u,v \in V_t}} w_{uv}\cdot\ONE \left(u \in S_t, v\in S_t\right).
\end{align*}

We charge the constraints violated at step $t$ of the algorithm to the LP weight of the edges removed at step $t$, which we denote by $LP_t$. Then,
\begin{align*}
LP_t =& \sum_{\substack{(u,v) \in E^+\\u,v \in V_t}} w_{uv} x_{uv} \cdot \ONE(u \in S_t \text{ or } v \in S_t)\\
&+ \sum_{\substack{(u,v) \in E^-\\u,v \in V_t}} w_{uv} (1 - x_{uv}) \cdot \ONE(u \in S_t \text{ or } v \in S_t)
\end{align*}

Note that the cost of the solution produced by the algorithm is the total weight of violations across all steps, that is $ALG = \sum\limits_t ALG_t$. Moreover, as every edge is removed exactly once from the graph, we can see that $LP = \sum\limits_t LP_t$. Hence, if we can show that $\mathbb{E}[ALG_t] \leq \rho \mathbb{E}[LP_t]$ for every step $t$, then we can conclude that the approximation factor of the algorithm is at most $\rho$ as,
$$
\mathbb{E}[ALG] = \mathbb{E}\bigg[\sum_t ALG_t \bigg] \leq \rho \cdot \mathbb{E}\bigg[\sum_t LP_t \bigg] =  \rho LP
$$

For analysis, we assume that each vertex $u$, has a positive (similar) self-loop, thus $cost(u,u\given w)=lp(u,u \given w) = 0$.

We now write $\mathbb{E}[ALG_t]$ and $\mathbb{E}[LP_t]$ in terms of $cost(\cdot)$ and $lp(\cdot)$ which are defined in Section~\ref{triple_Analysis}.
\begin{align}\label{ALGcost1}
\mathbb{E}[ALG_t \given V_t] =& \sum_{\substack{(u,v) \in E\\u,v \in V_t}} \bigg( \frac{1}{|V_t|} \sum_{w \in V_t} w_{uv} cost(u,v\given w)\bigg)\nonumber\\
=& \frac{1}{2|V_t|}\sum_{\substack{u,v,w \in V_t \\ u \neq v}} w_{uv} cost(u,v\given w)
\end{align}

\begin{align}\label{LPcost1}
\mathbb{E}[LP_t \given V_t] =& \sum_{\substack{(u,v) \in E\\u,v \in V_t}} \bigg( \frac{1}{|V_t|} \sum_{w \in V_t} w_{uv} lp(u,v\given w)\bigg)\nonumber\\
=& \frac{1}{2|V_t|}\sum_{\substack{u,v,w \in V_t \\ u \neq v}} w_{uv} lp(u,v\given w)
\end{align}

We divide the expressions on the right hand side by $2$ because the terms $cost(u,v \given w)$ and $lp(u,v \given w)$ are counted twice. Now adding the terms $cost(u,u \given w)$ and $lp(u,u \given w)$ (both equal to $0$) to~(\ref{ALGcost}) and~(\ref{LPcost}) respectively and grouping the terms containing $u,v$ and $w$ together, we get,
\begin{align*}
\mathbb{E}[ALG_t \given V_t] =& \frac{1}{6|V_t|}\sum_{u,v,w \in V_t}\bigg( w_{uv} cost(u,v\given w)\\
&+ w_{uw} cost(u,w\given v) + w_{wv} cost(w,v\given u)\bigg)\\
=&\frac{1}{6|V_t|}\sum_{u,v,w \in V_t} ALG^\sigma(x,y,z)
\end{align*}
and
\begin{align*}
\mathbb{E}[LP_t \given V_t] =& \frac{1}{6|V_t|}\sum_{u,v,w \in V_t}\bigg(w_{uv} lp(u,v\given w)\\
&+ w_{uw} lp(u,w\given v) + w_{wv} lp(w,v\given u)\bigg)\\
=&\frac{1}{6|V_t|}\sum_{u,v,w \in V_t}LP^\sigma(x,y,z)
\end{align*}


Thus, if $ALG^\sigma(x,y,z) \leq \rho LP^\sigma(x,y,z)$ for all signatures $\sigma$ and edge lengths $x,y,z$ satisfying the triangle inequality, then $\mathbb{E}[ALG_t] \leq \rho \cdot \mathbb{E}[LP_t]$, and, hence, $\mathbb{E}[ALG] \leq \rho \cdot \mathbb{E}[LP]$ which finishes the proof.

\end{proof} 
